Coordinate Invariant User-Guided Constrained Path Planning with Reactive Rapidly Expanding Plane-Oriented Escaping Trees

As collaborative robots move closer to human environments, motion generation and reactive planning strategies that allow for elaborate task execution with minimal easy-to-implement guidance whilst coping with changes in the environment is of paramount importance. In this paper, we present a novel approach for generating real-time motion plans for point-to-point tasks using a single successful human demonstration. Our approach is based on screw linear interpolation,which allows us to respect the underlying geometric constraints that characterize the task and are implicitly present in the demonstration. We also integrate an original reactive collision avoidance approach with our planner. We present extensive experimental results to demonstrate that with our approach,by using a single demonstration of moving one block, we can generate motion plans for complex tasks like stacking multiple blocks (in a dynamic environment). Analogous generalization abilities are also shown for tasks like pouring and loading shelves. For the pouring task, we also show that a demonstration given for one-armed pouring can be used for planning pouring with a dual-armed manipulator of different kinematic structure.

==> relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}
The basic approach to make robots autonomous for a particular task is hand-engineering of a controller. Yet the generalization of this task across the workspace is extremely hard \cite{kragic}. In previous works we have shown how screw linear interpolation (ScLERP) can be used for point-to-point path planning, in the context of respecting task-space motion constraints.
\subsection{Point to Point Trajectory generation}
\subsection{User-Guided Motion Planning}
\subsection{Reactive Obstacle Avoidance in the context of p2p planning}
